Definition of dose rate for FLASH pencil-beam scanning proton therapy: A comparative study

Purpose: Highlight the distinctions, both in terms of concept and numerical values, of the various definitions that can be established for the dose rate in PBS proton therapy. Methods: In an in silico study, five definitions of the dose rate, namely the PBS dose rate, the percentile dose rate, the maximum percentile dose rate, the average dose rate, and the dose averaged dose rate (DADR) were analyzed first through theoretical comparison, and then applied to a head and neck case. To carry out this study, a treatment plan utilizing a single energy level and requiring the use of a patient-specific range modulator was employed. The dose rate values were compared both locally and by means of dose rate volume histograms (DRVHs). Results: The PBS dose rate, the percentile dose rate, and the maximum percentile dose are definitions that are specifically designed to take into account the time structure of the delivery of a PBS treatment plan. Although they may appear similar, our study shows that they can vary locally by up to 10%. On the other hand, the DADR values were approximately twice as high as those of the PBS, percentile and maximum percentile dose rates, since the DADR disregards the periods when a voxel does not receive any dose. Finally, the average dose rate can be defined in various ways, as discussed in this paper. The average dose rate is found to be lower by a factor of approximately 1/2 than the PBS, percentile and maximum percentile dose rates. Conclusions: We have shown that using different definitions for the dose rate in FLASH proton therapy can lead to variations in calculated values ranging from a few percent to a factor of two. Since the dose rate is a critical parameter in FLASH radiation therapy, it is essential to carefully consider the choice of definition. However, to make an informed decision, additional biological data and models are needed.

==> old_tables.tex <==
\begin{table}
\centering
\caption{Percentile dose rates}
\begin{tabular}{lrrrrr}
\toprule
{} &   DR2 &   DR5 &  DR50 &  DR95 &  DR98 \\
\midrule
PTV 95           & 98.51 & 82.76 & 43.14 & 33.68 & 31.44 \\
PTV extension 95 & 96.87 & 84.48 & 31.05 &  3.76 &  2.37 \\
PTV 98           & 78.68 & 68.14 & 38.44 & 30.44 & 28.59 \\
PTV extension 98 & 77.56 & 68.40 & 27.31 &  3.39 &  2.10 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{PBS dose rates}
\begin{tabular}{lrrrrr}
\toprule
{} &   DR2 &   DR5 &  DR50 &  DR95 &  DR98 \\
\midrule
PTV 95           & 73.88 & 63.62 & 38.58 & 31.24 & 29.38 \\
PTV extension 95 & 73.93 & 65.94 & 29.51 &  5.41 &  3.85 \\
PTV 98           & 64.37 & 56.17 & 35.37 & 28.72 & 27.21 \\
PTV extension 98 & 62.81 & 56.50 & 26.10 &  4.16 &  2.84 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Relative threshold PBS dose rates}
\begin{tabular}{lrrrrr}
\toprule
{} &   DR2 &   DR5 &  DR50 &  DR95 &  DR98 \\
\midrule
PTV 95           & 83.40 & 71.03 & 41.37 & 32.47 & 30.24 \\
PTV extension 95 & 81.95 & 71.95 & 28.94 &  3.49 &  2.16 \\
PTV 98           & 70.68 & 60.78 & 37.20 & 29.64 & 27.87 \\
PTV extension 98 & 68.11 & 60.54 & 25.89 &  3.13 &  1.97 \\
\bottomrule
\end{tabular}
\end{table}

